Adapted Multimodal BERT with Layer-wise Fusion for Sentiment Analysis

Multimodal learning pipelines have benefited from the success of pretrained language models. However, this comes at the cost of increased model parameters. In this work, we propose Adapted Multimodal BERT (AMB), a BERT-based architecture for multimodal tasks that uses a combination of adapter modules and intermediate fusion layers. The adapter adjusts the pretrained language model for the task at hand, while the fusion layers perform task-specific, layer-wise fusion of audio-visual information with textual BERT representations. During the adaptation process the pre-trained language model parameters remain frozen, allowing for fast, parameter-efficient training. In our ablations we see that this approach leads to efficient models, that can outperform their fine-tuned counterparts and are robust to input noise. Our experiments on sentiment analysis with CMU-MOSEI show that AMB outperforms the current state-of-the-art across metrics, with 3.4% relative reduction in the resulting error and 2.1% relative improvement in 7-class classification accuracy.

==> Figures/adapters_ft.tex <==
\begin{table}[t!]
  \centering
  \small
%   \begin{tblr}{ |p{2.5cm, c}||p{1.4cm, c}|p{1.4cm, c}||p{2cm, c}|}
\begin{tblr}{|c|c|c|c|}
    \hline
    % \SetCell[c=4]{c}{{{Adapters vs Fine-tuning}}}\\\hline
     Models & Corr $(\uparrow)$ &  Acc-7 $(\uparrow)$ &  Train. Parameters \\\hline
    
    MISA-Adapters &  $0.758$ & $52.15$ & $8.5$\\ %$8,543,377$\\
    MISA & $0.756$ & $52.20$ & $47.1$\\ %47,124,625\\
    \hline
    AMB no-text & $0.240$ & $41.64$   & $8.6$\\ %8,593,231 \\ 
    AMB text-only &  $0.760$ & $52.81$ & $8.6$\\ %8,593,231 \\

 \hline 
    AMB-FT & $0.756$ & $51.98$ & $47.2$\\ %47,174,479 \\
    % AMB-LN & 0.7635 & 52.79 & 8,631,631 \\
    \textbf{AMB}  & $\mathbf{0.766}$ & $\mathbf{53.29}$ & $8.6$ \\ %8,593,231 \\
 \hline
  \end{tblr}
  \newline\newline
  \caption{Multimodal adapters vs fine-tuning. We include experiments, where the text, or the audio-visual modalities are missing. Trainable parameter are in millions.}\label{tab1}
\end{table}


==> Figures/plots.tex <==
\begin{figure*}[h!]
\begin{multicols}{2}
        \begin{subfigure}{0.4\textwidth}
            \input{Figures/plots/deleting_words}
            \caption{Randomly deleting words from input text}
            \label{fig:delete}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.4\textwidth}
            \input{Figures/plots/replacing_words}
            % \hfill
            \caption{Randomly replacing words from input text}
            \label{fig:replace}
        \end{subfigure}
    \end{multicols}
\begin{multicols}{2}
        \begin{subfigure}{0.4\textwidth}
        \input{Figures/plots/visual}
        % \hfill
        \caption{Injecting noise to visual modality}
        \label{fig:visual}
    \end{subfigure}
        \begin{subfigure}{0.4\textwidth}
            \input{Figures/plots/acoustic}
            % \hfill
            \caption{Injecting noise to acoustic modality}
            \label{fig:acoustic}
        \end{subfigure}
    \end{multicols}
\caption{Robustness Results}
\end{figure*}

==> Figures/plots/acoustic.tex <==
\begin{tikzpicture}[scale=0.75]

\begin{semilogxaxis}[
	xlabel={Noise Insertion Rate},
	ylabel={Correlation Coefficient},
% 	ymin=0.75,
%     ymax=77,
%  	extra y ticks{ 0.7645, 0.7575, 0.7565},
	ymajorgrids,
	anchor=north west,
% 	legend pos= outer north east,
	yticklabel style={/pgf/number format/fixed,
                  /pgf/number format/precision=3}
]

% MISA
\addplot[color=red, mark=triangle,] coordinates{
        (0.00001,0.7595)
        (0.00005,0.7595)
        (0.00010,0.7595)
        (0.00050,0.7595)
        (0.00100,0.7595)
        (0.00500,0.7595)
        (0.01000,0.7595)
        (0.05000,0.7595)
        (0.10000,0.7596)
        (0.20000,0.7597)
        (0.30000,0.7594)
        (0.40000,0.7593)
        (0.50000,0.7599)
        (1.00000,0.7600)
};
% \addlegendentry{$L/D$=2.5};
\addplot[color=blue, mark=o,] coordinates{
        (0.00001,0.7668)
        (0.00005,0.7668)
        (0.00010,0.7668)
        (0.00050,0.7668)
        (0.00100,0.7668)
        (0.00500,0.7668)
        (0.01000,0.7668)
        (0.05000,0.7668)
        (0.10000,0.7668)
        (0.20000,0.7668)
        (0.30000,0.7668)
        (0.40000,0.7668)
        (0.50000,0.7668)
        (1.00000,0.7668)
};

\addplot[color=green, mark=diamond,] coordinates{
    (0.00001,0.7562)
    (0.00005,0.7562)
    (0.00010,0.7562)
    (0.00050,0.7562)
    (0.00100,0.7562)
    (0.00500,0.7562)
    (0.01000,0.7562)
    (0.05000,0.7562)
    (0.10000,0.7562)
    (0.20000,0.7562)
    (0.30000,0.7562)
    (0.40000,0.7562)
    (0.50000,0.7562)
    (1.00000,0.7562)
};

% \legend{$MISA$,$AMB$,$AMB-FT$}
\end{semilogxaxis}

\end{tikzpicture}


==> Figures/plots/deleting_words.tex <==
\begin{tikzpicture}
\begin{semilogxaxis}[
    scale=0.8,
	xlabel={Probability of Deletion},
	ylabel={Correlation Coefficient},
	extra y ticks={0.085,  0.15, 0.2, 0.3, 0.5, 0.7, 0.76},
	yticklabel style={/pgf/number format/fixed,
	                /pgf/number format/precision=3},
	ymajorgrids,
	anchor=north west,
	legend pos= south west%outer north east
% 	xmajorgrids
]
% 	\draw[blue] \pgfextra{
% 	  \pgfpathellipse{\pgfplotspointaxisxy{0}{0}}
% 		{\pgfplotspointaxisdirectionxy{1}{1}}
% 		{\pgfplotspointaxisdirectionxy{0}{2}}
% 	};
% 	\addplot [mark={text}, text mark={MISA}] coordinates { (0.1,0.1) };
% \draw[color=red, mark={MISA},] coordinates{
%         (0.1,0.7595)
% };
% MISA
\addplot[color=red, mark=triangle,] coordinates{
        (0.00001,0.7592)    (0.00005,0.7594)
        (0.00010,0.7591)    (0.00050,0.7576)    (0.00100,0.7550)
        (0.00500,0.7343)    (0.01000,0.7084)    (0.05000,0.5075)    
        (0.10000,0.3238)    (0.20000,0.1588)    (0.30000,0.1222)
        (0.40000,0.1074)    (0.50000,0.1072)    (1.00000,0.1072)
};
% \addlegendentry{$L/D$=2.5};
\addplot[color=blue, mark=o,] coordinates{
    (0.00001,0.7668)   (0.00005,0.7662)   
    (0.00010,0.7664)   (0.00050,0.7627)   (0.00100,0.7606)   
    (0.00500,0.7359)   (0.01000,0.6996)   (0.05000,0.5236)   
    (0.10000,0.3489)   (0.20000,0.1953)   (0.30000,0.1576)   
    (0.40000,0.1545)   (0.50000,0.1546)   (1.00000,0.1546)   
};

\addplot[color=green, mark=diamond,] coordinates{
    (0.00001,0.7558)
    (0.00005,0.7557)
    (0.00010,0.7552)
    (0.00050,0.7505)
    (0.00100,0.7487)
    (0.00500,0.7182)
    (0.01000,0.6825)
    (0.05000,0.4717)
    (0.10000,0.2975)
    (0.20000,0.1417)
    (0.30000,0.1006)
    (0.40000,0.0846)
    (0.50000,0.0842)
    (1.00000,0.0842)
};

% \legend{$MISA$,$AMB$,$AMB-FT$}
\end{semilogxaxis}

\end{tikzpicture}


==> Figures/plots/replacing_words.tex <==
\begin{tikzpicture}

\begin{semilogxaxis}[
    % width=2\linewidth,
    % height=12cm,
    scale=0.8,
	xlabel={Probability of Replacement},
	ylabel={Correlation Coefficient},
	yticklabel style={/pgf/number format/fixed,
	                /pgf/number format/precision=3},
	extra y ticks={0.05, 0.1, 0.2, 0.3, 0.5, 0.7, 0.76},
	ymajorgrids,
	anchor=north west,
	legend pos= south west% outer north east
% 	xmajorgrids
]
% MISA
\addplot[color=red, mark=triangle,] coordinates{
    (0.00001,0.7595)
    (0.00005,0.7584)
    (0.00010,0.7583)
    (0.00050,0.7545)
    (0.00100,0.7505)
    (0.00500,0.7187)
    (0.01000,0.6720)
    (0.05000,0.3990)
    (0.10000,0.2142)
    (0.20000,0.0485)
    (0.30000,0.0271)
    (0.40000,0.0163)
    (0.50000,0.0290)
    (1.00000,0.0210)
};
% \addlegendentry{$L/D$=2.5};
\addplot[color=blue, mark=o,] coordinates{
    (0.00001,0.7668)
    (0.00005,0.7663)
    (0.00010,0.7664)
    (0.00050,0.7622)
    (0.00100,0.7607)
    (0.00500,0.7284)
    (0.01000,0.6886)
    (0.05000,0.4571)
    (0.10000,0.2499)
    (0.20000,0.0745)
    (0.30000,0.0459)
    (0.40000,0.0373)
    (0.50000,0.0462)
    (1.00000,0.0491)
};

\addplot[color=green, mark=diamond,] coordinates{
    (0.00001,0.7560)
    (0.00005,0.7560)
    (0.00010,0.7558)
    (0.00050,0.7514)
    (0.00100,0.7468)
    (0.00500,0.7075)
    (0.01000,0.6732)
    (0.05000,0.4150)
    (0.10000,0.2058)
    (0.20000,0.0490)
    (0.30000,0.0014)
    (0.40000,0.0102)
    (0.50000,0.0058)
    (1.00000,-0.0017)
};

\legend{$MISA$,$AMB$,$AMB-FT$}
\end{semilogxaxis}

\end{tikzpicture}


==> Figures/plots/visual.tex <==
\begin{tikzpicture}[scale=0.75]

\begin{semilogxaxis}[
	xlabel={Noise Insertion Rate},
	ylabel={Correlation Coefficient},
% 	ymin=0.75,
%     ymax=77,
%  	extra y ticks{ 0.7645, 0.7575, 0.7565},
	ymajorgrids,
	anchor=north west,
% 	legend pos= outer north east,
	yticklabel style={/pgf/number format/fixed,
                  /pgf/number format/precision=3}
]

% MISA
\addplot[color=red, mark=triangle,] coordinates{
    (0.00001,0.7595)
    (0.00005,0.7595)
    (0.00010,0.7595)
    (0.00050,0.7595)
    (0.00100,0.7595)
    (0.00500,0.7595)
    (0.01000,0.7595)
    (0.05000,0.7595)
    (0.10000,0.7593)
    (0.20000,0.7594)
    (0.30000,0.7587)
    (0.40000,0.7593)
    (0.50000,0.7592)
    (1.00000,0.7572)
};
% \addlegendentry{$L/D$=2.5};
\addplot[color=blue, mark=o,] coordinates{
    (0.00001,0.7668)
    (0.00005,0.7668)
    (0.00010,0.7668)
    (0.00050,0.7668)
    (0.00100,0.7668)
    (0.00500,0.7668)
    (0.01000,0.7668)
    (0.05000,0.7668)
    (0.10000,0.7669)
    (0.20000,0.7664)
    (0.30000,0.7663)
    (0.40000,0.7662)
    (0.50000,0.7659)
    (1.00000,0.7645)
};

\addplot[color=green, mark=diamond,] coordinates{
    (0.00001,0.7562)
    (0.00005,0.7562)
    (0.00010,0.7562)
    (0.00050,0.7562)
    (0.00100,0.7562)
    (0.00500,0.7562)
    (0.01000,0.7562)
    (0.05000,0.7562)
    (0.10000,0.7562)
    (0.20000,0.7562)
    (0.30000,0.7562)
    (0.40000,0.7562)
    (0.50000,0.7562)
    (1.00000,0.7562)
};

% \legend{$MISA$,$AMB$,$AMB-FT$}
\end{semilogxaxis}

\end{tikzpicture}


